Human Intention Estimation based on Hidden Markov Model Motion Validation for Safe Flexible Robotized Warehouses

With the substantial growth of logistics businesses the need for larger warehouses and their automation arises, thus using robots as assistants to human workers is becoming a priority. In order to operate efficiently and safely, robot assistants or the supervising system should recognize human intentions in real-time. Theory of mind (ToM) is an intuitive human conception of other humans' mental state, i.e., beliefs and desires, and how they cause behavior. In this paper we propose a ToM based human intention estimation algorithm for flexible robotized warehouses. We observe human's, i.e., worker's motion and validate it with respect to the goal locations using generalized Voronoi diagram based path planning. These observations are then processed by the proposed hidden Markov model framework which estimates worker intentions in an online manner, capable of handling changing environments. To test the proposed intention estimation we ran experiments in a real-world laboratory warehouse with a worker wearing Microsoft Hololens augmented reality glasses. Furthermore, in order to demonstrate the scalability of the approach to larger warehouses, we propose to use virtual reality digital warehouse twins in order to realistically simulate worker behavior. We conducted intention estimation experiments in the larger warehouse digital twin with up to 24 running robots. We demonstrate that the proposed framework estimates warehouse worker intentions precisely and in the end we discuss the experimental results.

==> VR_warehouse.tex <==
\section{Overview of the Virtual Reality Setup}
We built a VR framework for rapid prototyping of components in the project SafeLog (specifically AR), a tool that might also evolve into a training framework in the future. The main reason behind it is that the large commercial automated warehouses are unavailable for testing, yet it is important to do tests in full scale warehouses to identify potential problems. This also enables us to do tests with multiple users more freely as to get the best interaction modalities as possible. The application currently runs in \textit{Unity3D 2017.1.2} and is used with the \textit{HTC Vive} headset. \par
The warehouses layout is planned using Swisslog's network planner. Once the layout is done an xml file is exported. The file can then be parsed by our program which, together with available CAD models, builds the VR warehouse from scratch. The fleet of robots is presently controlled by parsing a series of JSON messages stored in a text file. These messages are the output of the Path planner developed by our partners at CVUT. Since the path planner and interfaces are still work in progress this was chosen as the most direct method. As an addition, an A* algorithm was implemented for the navigation of the user. An additional pseudo-random motion algorithm has been implemented for robot movement. The robot is positioned on one of the navigation nodes at random. It selects one of the reachable adjacent nodes also at random. It then continues selecting nodes in such a manner except that it is not allowed to return to the node visited in the previous step, and if another robot already selected the same node in the same time step, it stops and waits for it to pass. This works well at emulating a fleet of robots moving around the warehouse without collisions. \par
For the prototyping of AR interactions, path visualization and picking assistance have been implemented. The VR setup emulates the Hololens - all of the "holographic objects" are only visible through a narrow field of view (FoV) as in the Microsoft Hololens, which has a, depending on the specs one reads, 30\degree{} to 35\degree{} Horizontal and 17.5\degree{} to 17.82\degree{} Vertical FoV. In the simulation we use the lower estimates. The pointer is also taken directly from the Hololens and uses raycasting to position itself on objects. \par     
Such a system allows us for example to test if a certain interaction modalities fails or is not as informative because of the low FoV in a realistic environment. It also allows us to inject localization errors to determine at witch point the various interaction modalities becomes unusable. \par
Future works includes full communication with the path planner, integration of more AR interactions, integration of multiuser support and evaluation of the feasibility to further develop it into a training tool. \par   

==> experiments_AR_VR.tex <==
\subsection{Experiments with AR}
The experiments were conducted in the laboratory of our project partner Swisslog in Ettlingen, with twelve racks and two robots. The layout is visible in Fig.\ref{laboratory_layout}. Although small scale, it presented an opportunity for testing in a realistic environment. We used the Hololens' inbuilt localization algorithm to follow the person while walking inside the warehouse. Since no external tracker was used, the person started from a predefined ground node (R32 in Fig.\ref{laboratory_layout}) and then walked from ground node to ground node, in a similar fashion to the robots. All AR interactions were disabled and the person navigated the warehouse autonomously. The only exception being that a holographic sphere was positioned at the Hololens' location every 100 frames. This allowed us, together with the walking modality of the human, to also conduct a qualitative analysis of the localization, since no quantitative analysis was yet conducted on the device. This showed that the localization was indeed robust with only a few centimeter deviation at most from the straight line paths between nodes. The deviation however could also be explained by imperfect walking of the user from node to node, increasing the accuracy even further. \par
In total, five tests were made, the first one without robots, purely to evaluate the robustness in a warehouse-like environment, and then two tests per scenarios. The scenarios themselves altered the goal of the user and the path of the mobile robot. In the first scenario the user needed to reach node R109, however a stationary robot was positioned at R15 and another robot would start moving forward from node R107 as soon as the person reached the node R7. In the second scenario the person wants to reach the node R108 and then proceed to node R16. Once the person reaches the R108 node, a robot starts moving forward from node R105, requiring the user to backtrack and approach from the other side. The stationary robot  was nce again placed on node R15 as an obstacle.      
\subsection{Experiments with VR}
Due to the lack of access to a full-scale warehouse for testing, we did a second round of larger-scale tests in VR, using the system already described in the previous section. The tracking of the HTC Vive has a RMS error of 1.9mm. We tracked the position of the user, as well as each of the robot. \par
As a proof of concept, we first did four tests with the same setup as the AR experiment, see Fig\ref{AR_VR}. We then proceeded to do another batch of four tests, where we used a small test warehouse (Fig.\ref{small_layout}) with four robots running on preprogrammed paths. These paths were generated by the path planner and read from a text file containing JSON messages. Each of the four tests had a different goal. \par 
Another nine tests were made on the small-scale test warehouse with 24 robots. The robots were placed in groups of eight on the far left, middle and far right vertical corridors, equally spaced vertically. The first four tests were deterministic, where the robots select the first adjacent node on the list except for the node it came from. This creates a cyclic, predefined motion of the robots, meaning that after the first few experiments the user knew approximately how the robots would move. The next five tests were made with the pseudo-random motion as described in the VR Setup section. With this motion model, the user isn't able to predict the motions of the robots (though there are one-way corridors where the motion can then be predicted). In the last of the tests the user didn't have a predetermined goal and was just walking around, trying to avoid robots.     

\begin{figure}[ht!]
	\centering
	\includegraphics[width=0.47\textwidth]{figures/laboratory.jpg}
	\caption{The layout of the Laboratory in Ettlingen, used for AR-based experiments}
	\label{laboratory_layout}
\end{figure}

\begin{figure}[ht!]
	\centering
	\includegraphics[width=0.47\textwidth]{figures/smallCarryPick.pdf}
	\caption{The small warehouse layout, used for VR-based experiments}
	\label{small_layout}
\end{figure}

\begin{figure*}[b]
\centering
\subfloat[First-person view from the 2 Megapixel Hololens camera\label{AR_exp}]{\includegraphics[width=0.45\textwidth]{figures/AR_ett.png}}
\subfloat[First-person view from HTC Vive\label{VR_exp}]{\includegraphics[width=0.46\textwidth]{figures/VR_ett.png}}
\caption{Comparison between the real-world experiment and the experiments in VR. Both experiments use exactly the same setup.}
\label{AR_VR}
\end{figure*}




==> intro_VR_AR.tex <==
Augmented reality (AR) and virtual reality (VR) have seen a big resurgence in robotics in the recent years \cite{Williams2018VAMHRI}, mostly due to the recent availability of off-the-shelf commercial products. Here we give a brief overview of the history and recent use of both technologies in the fields of robotics, manufacturing and logistics. \par
Virtual reality refers to systems where the input from the outside world is totally blocked and replaced by system-generated input. The first VR system was built in 1968 by Ivan Sutherland \cite{Sutherland1968Damocles}. The device was extremely bulky and the screen resolution poor, however it proved that VR is achievable. The first usable VR system came in 1992 with the CAVE system by Cruz-Neira et al. \cite{CruzNeira1992CAVE}. The CAVE is a special room where electromagnetic (now infrared) trackers track the 3D glasses (now usually with active polarization) and projectors display the appropriate images on the room's surfaces. Although viable as a system, especially for prototyping \cite{Seth2011VRPrototyping}, it was not flexible enough to be widely employed, requiring expensive sensors and a purposely designed room. \par Advancements in VR technology have seen the CAVE systems of the early 90s being replaced by cheaper and more flexible headsets such as the \textit{Oculus Rift} or the \textit{HTC Vive}. This has sparked a boom in the field of robotics where VR has recently seen the most use as a more intuitive method for teleoperation of stationary \cite{Lipton2018VRBaxter}, mobile \cite{Jankowski2015VRMobileRobot} and humanoid robots \cite{allspaw2018remotely}. A natural extension of such a teleoperation systems is a more immersive tool for telepresence robots \cite{Zhang2018telepresence}. It has also emerged as a method to teach virtual robots how to preform tasks \cite{Zhang2017VRDL}. The knowledge is then successfully transfered to a real robot. In manufacturing \cite{Mujeber2004VRManufacturing} VR has seen use as a virtual prototyping \cite{CHOI2004VirtualPrototyping} and training tool \cite{gavish2015evaluating}. As a training tool, VR has proven to increase performance of trainees in other areas as well, such as medicine \cite{seymour2002virtual} and safety training in construction \cite{sacks2013construction} and mining \cite{squelch2001virtual}. \par
Augmented reality, in contrast to VR, seeks to add information to the input from the real world. The first AR systems started to appear in the 80s, mostly for military research. The most commonly quoted first functional AR system was the \textit{Virtual Fixtures} system \cite{rosenberg1992use}, developed in 1992 by Louis Rosenberg for the US Air Force. Quickly it's usefulness became apparent in other fields as well, such as manufacturing, medicine, entertainment and robotics, where the first use cases focused on assistance in robotic teleoperation via a stereo camera pair \cite{Milgram1993HumanRobotCommunication}. These first AR systems in robotics added data to a camera stream and displayed the enhanced view on computer monitors \cite{bischoff2004perspectives}. Today's AR can be mostly divided into projector based, tablet/smartphone based, head mounted and computer screen based, with the last one becoming less popular. \par
Projector based AR has seen use for visualizing robot's intentions and intuitive programming of robots in robot work cells \cite{gaschler2014intuitive}, displaying intentions of mobile robots operating in human environments \cite{Chadalavada2015thats}, as well as for debugging and rapid prototyping of robotic systems through visualization of sensor data \cite{omidshafiei2016ARPrototyping}. \par
Tablets have seen use in AR-assisted robot programming \cite{mateo2014hammer}. Devices like the \textit{Google Tango} tablet, in addition, with inbuilt Simultaneous Localization and Mapping (SLAM), \cite{Cadena2016SLAMSurvey} can be used for markerless AR applications. The main problem with tablets is that it occupies the hands, preventing any work while the AR information is visualized. With the recent releases of the ARCore and ARKit toolkits, for Android and iOS devices respectively, tablet and smartphone based AR applications are becoming a cheap and straightforward interaction modality for home robots \cite{Sprute2017VirtualBorders}. \par
Head mounted systems can be further divided into Heads-up Display (HUD) systems and "Full-AR" systems, with the most famous member of the former being the \textit{Google Glass} and of the later \textit{Microsoft Hololens}. As the name implies HUD-based systems don't have any advanced localization or computing systems and therefore are only able to display HUD interfaces, while Full-AR systems are able to perform inside-out localization using SLAM and display persistent, fully 3D holograms in space. HUD systems have found success in logistics, where they have been used for "pick-by-vision" systems to quicken and ease the picking of items in warehouses \cite{Schwerdtfeger2011PickByVision}. Since full-AR systems, starting with the \textit{Hololens}, haven't been on the market for long, research is just starting \cite{Williams2018VAMHRI}, with the most prominent field perhaps being AR-assisted robot programming \cite{Guhl2017Hololens}. \par
In the SafeLog project we use the VR environment mostly for rapid prototyping and testing of AR interactions, while in the future it should be easily expanded for training purposes and possibly system monitoring. The AR interactions are developed for the \textit{Microsoft Hololens} and build upon the standard use of AR in logistics as part of "pick-by-vision" systems to include navigational help, situational awareness and maintenance help for humans working in a mostly automated warehouse. In addition using a Head-mounted device allows the user to perform any manual task unimpeded. The robust localization and sensors of such devices also provides opportunities for Human Intention Recognition, as described in this article.  \par 

